Self-Confirming Equilibrium under Model Misspecification

We study the steady states of games played recurrently within large anonymous populations of players who receive partial ex-post feedback about the play of their opponents. Departing from the classical Bayesian account, players do not trust their conjectures as a correct description of the strategic environment but consider them as approximations of a reality that is only partially modeled and partially observed. We introduce games with feedback and uncertainty attitudes, in which the normal-form structure is enriched with a profile of feedback functions and, for each player, a preference functional that encodes aversion to misspecification and to ambiguity. The induced misspecification sensitive criterion contains the variational, maxmin, and smooth-ambiguity evaluations as special cases and collapses to expected utility when beliefs are unambiguous and the player is neutral to misspecification. The appropriate steady-state notion for such games is the Self-Confirming Equilibrium under Model Misspecification (SCEM), which requires each player to best respond to a set of structured conjectures that the feedback generated by equilibrium play cannot falsify. In contrast with the classical theory and with its ambiguity-averse extensions, mixed-strategy Nash Equilibria need not be self-confirming. We therefore develop a companion notion of Robust Nash Equilibrium (R-NE), in which every supported action remains optimal under a variational evaluation. Robust Nash equilibria refine SCEM, exist whenever the statistical distances are continuous, thereby delivering existence of SCEM, and coincide with the latter under fully informative feedback. Under observationally consistent divergences and observable payoffs, R-NE and SCEM reduce, respectively, to Nash equilibrium and Self-Confirming Equilibrium under Ambiguity (SCEA), which generalizes smooth self-confirming equilibrium.

==> Makefile <==
# partly autogenerated, that's why it's so ugly!

# say 'make V=1' to see the full build output
ifndef V
Q = @
Q_LATEX = sh -c 'echo -e "   " `echo $$(basename "$$0") | tr a-z A-Z`"\t$${!\#/..\/..\//}"; ! "$$0" "$$@" | grep -A5 -E "^[^ ]+:[0-9]+:"'
Q_OTHER = sh -c 'echo -e "   " `echo $$(basename "$$0") | tr a-z A-Z`"\t$${!\#/..\/..\//}"; "$$0" "$$@" >/dev/null'
endif

LATEX = latex
PDFLATEX = pdflatex
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOEPS = pdftops -eps
PDFTOPS = pdf2ps
EPSTOPDF = epstopdf
FIGTODEV = fig2dev
MPOST = mpost

.PHONY: all clean archive

all:  thesis

texfiles = $(wildcard *.tex)

.PHONY: thesis
thesis: thesis.pdf thesis.ps

thesis.pdf: $(texfiles) thesis.bbl
	$(Q) rm -rf build/pdf/; mkdir -p build/pdf/
	$(Q) cd build/pdf/ && TEXINPUTS="../../:$$TEXINPUTS" $(Q_LATEX) $(PDFLATEX) -interaction=nonstopmode -file-line-error ../../thesis.tex
	$(Q) cd build/pdf/ && TEXINPUTS="../../:$$TEXINPUTS" $(Q_LATEX) $(PDFLATEX) -interaction=nonstopmode -file-line-error ../../thesis.tex
	$(Q) ln -f build/pdf/thesis.pdf thesis.pdf

thesis.dvi: $(texfiles) thesis.bbl
	$(Q) rm -rf build/dvi/; mkdir -p build/dvi/
	$(Q) cd build/dvi/ && TEXINPUTS="../../:$$TEXINPUTS" $(Q_LATEX) $(LATEX) -interaction=nonstopmode -file-line-error ../../thesis.tex
	$(Q) cd build/dvi/ && TEXINPUTS="../../:$$TEXINPUTS" $(Q_LATEX) $(LATEX) -interaction=nonstopmode -file-line-error ../../thesis.tex
	$(Q) ln -f build/dvi/thesis.dvi thesis.dvi

thesis.ps: thesis.dvi
	$(Q)$(Q_OTHER) $(DVIPS) -q thesis

thesis.aux: $(texfiles)
	$(Q) $(Q_LATEX) $(LATEX) -interaction=nonstopmode -file-line-error thesis.tex

thesis.bbl: thesis.aux
	$(Q)$(Q_OTHER) $(BIBTEX) thesis

clean:
	rm -rf build/
	rm -f *.aux
	rm -f thesis.dvi thesis.idx thesis.ind thesis.ilg thesis.out thesis.toc thesis.pdf thesis.log

archive: thesis-template.zip

thesis-template.zip: *.tex Makefile ETHlogo.* refs.bib
	mkdir -p thesis
	cp `git ls-files "*.tex" Makefile "ETHlogo.*" refs.bib` thesis/
	perl -i -pe 's/\$$VERSION\$$/'"$$(git describe)/" thesis/*.tex
	rm -f thesis-template.zip
	zip -r thesis-template.zip thesis/

